Trust Your Robots! Predictive Uncertainty Estimation of Neural Networks with Sparse Gaussian Processes

This paper presents a probabilistic framework to obtain both reliable and fast uncertainty estimates for predictions with Deep Neural Networks (DNNs). Our main contribution is a practical and principled combination of DNNs with sparse Gaussian Processes (GPs). We prove theoretically that DNNs can be seen as a special case of sparse GPs, namely mixtures of GP experts (MoE-GP), and we devise a learning algorithm that brings the derived theory into practice. In experiments from two different robotic tasks -- inverse dynamics of a manipulator and object detection on a micro-aerial vehicle (MAV) -- we show the effectiveness of our approach in terms of predictive uncertainty, improved scalability, and run-time efficiency on a Jetson TX2. We thus argue that our approach can pave the way towards reliable and fast robot learning systems with uncertainty awareness.

==> chapters/experiments.tex <==
\section{Experiments}
\label{sec:experiments}

\textbf{Toy illustration}

\begin{itemize}
	\item Central question: to validate (i) whether our approach works in principle (theoretic justification), (ii) and also see the influence of patchwork prior, in that it reduces the discontinuity problem. 
	\item Set-up: Start with a small toy example, so that we gain more insight, where it is easy to control all the experimental variables. Use snelson. Trained a small network and small data-set. We leave certain section out and test-set covers also out-of-distribution. Whenever there is no data, we should see high uncertainty, and whenever there is data, we should see the data uncertainty. Try with and without patchwork prior.
	\item What we need: figures that show answering our central question. One figure showing the uncertainty, and other figure, showing the transformed space uncertainty, where discontinuity is more visible.
\end{itemize}

\textbf{Ablation Studies}

\begin{itemize}
	\item Central question: there are many hyperparameters in the approach, and we would like to know their influence on the performance. Specifically, (i) influence of number of experts, (ii) influence of subset for PCA, (iii), influence of post-hoc pruning, and (iv) targetted-pruning, and (v) active learning selection on the boundaries.
	\item Set-up: use sarcos data-set, and vary the settings over the chosen ranges. We then measure, testing time, mll, nll, rmse, train rmse etc in order to see their influence. Then, we select the measures that are meaningful per hyperparameter iterations. Rest to appendix, and remaining to here.
	\item What we need: figures that answers our question, and conclusion on each hyperparameters to our best. 
	\item Investigate also the time it takes to run using the distributed framework. 
\end{itemize}

\begin{figure*}
	\centering
	\includegraphics[width=1.0\linewidth]{figures/ablation.pdf}
	\caption{Ablation study.}
\label{fig:exp:ab}
\end{figure*}

\textbf{Application 1: Robot Inverse Dynamics Learning}

\begin{itemize}
	\item Central question: are we competitive over existing methods that are non-realtime or real-time but relying on uncertainty propagation? Are we fast as well? Baselines are competitive and motivate again, why these baselines are meaningful.
	\item Set-up: Train a network on sarcos, kuka 1, kuka 2, and kuka sim. We also test the OOD set-up as well, for evaluation. 
	\item What we need: a big table that answers the question, and conclusion on when our approach works, and when it doesnt.
\end{itemize}

\input{tables/table_inverse_dynamics}

\textbf{Application 2: Visual-Inertial Odometry}

\begin{itemize}
	\item Central question: are we competitive over existing methods that are non-realtime or real-time but relying on uncertainty propagation? Are we fast again? Difference is that we test on perception tasks, and see if similar findings hold. We also want to validate if our approach works over the perception tasks.
	\item Set-up: Train 3 networks on KITTI. Motivation for each architectures. Split the training and evaluation set. We not only test on the nominal set-up but also test the sensor degradation scenarios where we intentionally corrupt the images and also inertial data.
	\item What we need: a big table that answers the question, and conclusion on when our approach works, and when it doesnt.
\end{itemize}

\input{tables/table_vio}

\textbf{Real robot experiments}

\begin{itemize}
	\item Central question: can we run our framework on a real robot (a multicopter that only has a limited power resources?
	\item Set-up: We use object detection as a benchmark: (i) the approach works for classification, (ii) the approach works in real-time.
	\item Replace this with a video.
\end{itemize}

\textbf{Use case of the proposed approach}

\begin{itemize}
	\item Mention the benefits again: the 3 key benefits, and how it can be useful for robotics.
	\item Mention the limitation but also point out how to solve them: scalability for multioutput gp (one can leverage the recent advances in GP for high output dimension), and further reduction in computational complexity (GP distillation into a single smaller GP). 
	\item Mention the potential impact of our work or use-cases of our method: for smaller output dim, the approach works and can be very useful, that GP can provide uncertainty directly. 
\end{itemize}

==> chapters/experiments4.tex <==
\subsection{Application 2: Visual-Inertial Odometry}

In the following we demonstrate the effectiveness of our method with the second application of visual inertial odometry \cite{shinde2020learning}. 
In this task, we want to estimate the relative poses between the consecutive cameras based on frames of video sequences and the corresponding IMU data including accelerator and gyroscope data. 
The normal setting is to evaluate the average RMSE between the ground truth data and the predicted camera poses transformed from the predicted relative poses along the sequences. 
To note that our goal is to provide better uncertainty estimation instead of achieving best performance. 
For this purpose we measure the NLL of the predicted relative motions without any further transformation. 
The KITTI visual odometry dataset \citep{Geiger2012CVPR} is employed for evaluation, in which video sequences 03, 06, 07, 10 are used for testing while the others for training.
Similar to the experimental settings in robot inverse dynamic learning, we construct OOD scenarios for this task. 
Different to taking another dataset directly, we on purpose shift the training data distribution by corrupting the different sources of data (IMU and image) with operations such as adding noise, removing data points, partial occlusions and so on.
Therefore we have three more corresponding OOD datasets, which degrade the image data only, IMU data only and both image and IMU data, respectively. 
Three different network architectures including MHA \citep{shinde2020learning}, VINET\citep{conf/cvpr/ClarkWMTW17}, VIOSOFT\citep{chen2019selective} have been taken for performance comparison among our method and other baselines. 

The results are in table \ref{table:vio}.
We can see from the results that... 

% \begin{itemize}
% 	\item Central question: are we competitive over existing methods that are non-realtime or real-time but relying on uncertainty propagation? Are we fast again? Difference is that we test on perception tasks, and see if similar findings hold. We also want to validate if our approach works over the perception tasks.
% 	\item Set-up: Train 3 networks on KITTI. Motivation for each architectures. Split the training and evaluation set. We not only test on the nominal set-up but also test the sensor degradation scenarios where we intentionally corrupt the images and also inertial data.
% 	\item What we need: a big table that answers the question, and conclusion on when our approach works, and when it doesnt.
% \end{itemize}

\input{tables/table_vio} 
\footnote{There are two different ways to compute the NLL values for different methods of uncertainty estimation. One uses the predicted samples only while the other requires the moments such as predicted mean and variance. In the table we used the former for the baselines and latter for our method. More discussions are referred to the appendix \ref{NLL_discussion}.}

==> tables/table_vio.tex <==
\begin{table}[ht]
	\setlength{\tabcolsep}{0.3em}
	\centering
	\caption{\textbf{Visual-inertial odometry experiments} Results in NLL$^1$ (avg. over 6 DOF)}
	\begin{tabular}[ht]{lccccc}
		\toprule
		& \textbf{MC-dropout} & \textbf{rMC-dropout} & \textbf{Laplace} & \textbf{rLaplace} & \textbf{Ours}    \\
		\midrule
		\underline{\textit{VIOSOFT}}  \\
		nominal                       &    1.2663	        &    1.2663            &   1.2664         &   1.2665          &   0.0$\pm$0.0    \\
		vis. degr.                    &    1.2670	        &    1.2670	           &   1.2672         &   1.2672          &   0.0$\pm$0.0    \\
		imu degr.                     &    1.2664	        &    1.2664   	       &   1.2664         &   1.2665          &   0.0$\pm$0.0    \\
		both degr.                    &    1.2671           &    1.2672            &   1.2672         &   1.2672          &   0.0$\pm$0.0    \\
		\midrule
		\underline{\textit{VINET}}                                                                                                           \\
		nominal                       &    1.2672	        &    1.2671       	   &   1.2672         &   1.2672          &   0.0$\pm$0.0    \\
		vis. degr.                    &    1.2678      		&    1.2676       	   &   1.2678         &   1.2679          &   0.0$\pm$0.0    \\
		imu degr.                     &    1.2753	        &    1.2749		       &   1.2745         &   1.2746          &   0.0$\pm$0.0    \\
		both degr.                    &    1.2774      		&    1.2770		       &   1.2768         &   1.2767          &   0.0$\pm$0.0    \\
		\midrule
		\underline{\textit{MHA}}                                                                                                             \\
		nominal                       &    1.2664    		&    1.2663		       &   1.2663         &   1.2663          &   0.0$\pm$0.0    \\
		vis. degr.                    &    1.2667	      	&    1.2665		       &   1.2667         &   1.2667          &   0.0$\pm$0.0    \\
		imu degr.                     &    1.2664     		&    1.2663		       &   1.2664         &   1.2664          &   0.0$\pm$0.0    \\
		both degr.                    &    1.2667      		&    1.2665       	   &   1.2667         &   1.2667          &   0.0$\pm$0.0    \\
		\bottomrule
	\end{tabular}
	\label{table:vio}
\end{table}%


==> tables/table_vio_nll.tex <==
\begin{table}[ht]
	\setlength{\tabcolsep}{0.3em}
	\centering
	\caption{\textbf{Visual-inertial odometry experiments} Results in NLL\_moments (avg. over 6 DOF). Average runtime per architecture in milliseconds.}
	\begin{tabular}[ht]{lccccc}
		\toprule
		& \textbf{MC-dropout} & \textbf{rMC-dropout} & \textbf{Laplace} & \textbf{rLaplace} & \textbf{Ours}    \\
		\midrule
		\underline{\textit{VIOSOFT}}  &    0.0$\pm$0.0 ms   &    0.0$\pm$0.0 ms    &   0.0$\pm$0.0 ms &   0.0$\pm$0.0 ms  &   0.0$\pm$0.0 ms \\
		nominal                       &    0.5758	        &    0.5756            &   0.5759         &   0.5762          &   0.0$\pm$0.0    \\
		vis. degr.                    &    0.5784	        &    0.5785	           &   0.5788         &   0.5791          &   0.0$\pm$0.0    \\
		imu degr.                     &    0.5760	        &    0.5759   	       &   0.5759         &   0.5762          &   0.0$\pm$0.0    \\
		both degr.                    &    0.5785           &    0.5789            &   0.5789         &   0.5792          &   0.0$\pm$0.0    \\
		\midrule
		\underline{\textit{VINET}}    &    0.0$\pm$0.0 ms   &    0.0$\pm$0.0 ms    &   0.0$\pm$0.0 ms &   0.0$\pm$0.0 ms  &   0.0$\pm$0.0 ms \\
		nominal                       &    0.5792	        &    0.5789       	   &   0.5792         &   0.5793          &   0.0$\pm$0.0    \\
		vis. degr.                    &    0.5816      		&    0.5808       	   &   0.5816         &   0.5818          &   0.0$\pm$0.0    \\
		imu degr.                     &    0.6114	        &    0.6096		       &   0.6084         &   0.6085          &   0.0$\pm$0.0    \\
		both degr.                    &    0.6200      		&    0.6185		       &   0.6169         &   0.6169          &   0.0$\pm$0.0    \\
		\midrule
		\underline{\textit{MHA}}      &    0.0$\pm$0.0 ms   &    0.0$\pm$0.0 ms    &   0.0$\pm$0.0 ms &   0.0$\pm$0.0 ms  &   0.0$\pm$0.0 ms \\
		nominal                       &    0.5758    		&    0.5755		       &   0.5757         &   0.5757          &   0.0$\pm$0.0    \\
		vis. degr.                    &    0.5770	      	&    0.5762		       &   0.5769         &   0.5770          &   0.0$\pm$0.0    \\
		imu degr.                     &    0.5760     		&    0.5756		       &   0.5758         &   0.5759          &   0.0$\pm$0.0    \\
		both degr.                    &    0.5772      		&    0.5764       	   &   0.5771         &   0.5772          &   0.0$\pm$0.0    \\
		\bottomrule
	\end{tabular}
	\label{table:vio_nll}
\end{table}%

==> tables/table_vio_rmse.tex <==
\begin{table}[ht]
\setlength{\tabcolsep}{0.3em}
\centering
\caption{\textbf{Visual-inertial odometry experiments} Results in RMSE (avg. over 6 DOF).}
\begin{tabular}[ht]{lccccc}
\toprule
                              & \textbf{MC-dropout} & \textbf{rMC-dropout} & \textbf{Laplace} & \textbf{rLaplace} & \textbf{Ours}    \\
\midrule
\underline{\textit{VIOSOFT}}                                                                                                         \\
nominal                       &    0.0220	        &    0.02130            &   0.0233         &   0.0281          &   0.0$\pm$0.0    \\
vis. degr.                    &    0.0326	        &    0.0324	           &   0.0324         &   0.0398          &   0.0$\pm$0.0    \\
imu degr.                     &    0.0226	        &    0.0224   	       &   0.0235         &   0.0284          &   0.0$\pm$0.0    \\
both degr.                    &    0.0323           &    0.0324            &   0.0324         &   0.0402          &   0.0$\pm$0.0    \\
\midrule
\underline{\textit{VINET}}                                                                                                           \\
nominal                       &    0.0315	        &    0.0311       	   &   0.0310         &   0.0365          &   0.0$\pm$0.0    \\
vis. degr.                    &    0.0369      		&    0.0356       	   &   0.0353         &   0.0424          &   0.0$\pm$0.0    \\
imu degr.                     &    0.0983	        &    0.0964		       &   0.0920         &   0.0987          &   0.0$\pm$0.0    \\
both degr.                    &    0.1083      		&    0.1069		       &   0.1022         &   0.1092          &   0.0$\pm$0.0    \\
\midrule
\underline{\textit{MHA}}                                                                                                             \\
nominal                       &    0.0216    		&    0.0211		       &   0.0209         &   0.0245          &   0.0$\pm$0.0    \\
vis. degr.                    &    0.0259	      	&    0.0241		       &   0.0241         &   0.0296          &   0.0$\pm$0.0    \\
imu degr.                     &    0.0223     		&    0.0217		       &   0.0214         &   0.0250          &   0.0$\pm$0.0    \\
both degr.                    &    0.0264      		&    0.0250       	   &   0.0243         &   0.0303          &   0.0$\pm$0.0    \\
\bottomrule
\end{tabular}
\label{table:vio_rmse}
\end{table}%

